CREATIVESUMM: Shared Task on Automatic Summarization for Creative Writing

This paper introduces the shared task of summarizing documents in several creative domains, namely literary texts, movie scripts, and television scripts. Summarizing these creative documents requires making complex literary interpretations, as well as understanding non-trivial temporal dependencies in texts containing varied styles of plot development and narrative structure. This poses unique challenges and is yet underexplored for text summarization systems. In this shared task, we introduce four sub-tasks and their corresponding datasets, focusing on summarizing books, movie scripts, primetime television scripts, and daytime soap opera scripts. We detail the process of curating these datasets for the task, as well as the metrics used for the evaluation of the submissions. As part of the CREATIVESUMM workshop at COLING 2022, the shared task attracted 18 submissions in total. We discuss the submissions and the baselines for each sub-task in this paper, along with directions for facilitating future work in the field.

==> 6-ethics.tex <==
% \section{Ethical Considerations}
% \paragraph{Data Collection}
% All data described was collected exclusively for the academic purpose of conducting research.
% %
% The purpose of using the summaries and data was only for training the model and not for public display or any other use.
% %
% No data was stored upon completion of the research process.

% \paragraph{Data Biases}
% %
% The \DatasetName~dataset contains books written or translated into English. % and so the stories in them mainly represent the culture of the English speaking populace.
% %
% These books are also more than fifty years old and so representative of society in that era.
% %
% The various pretrained models we evaluated on our dataset carry biases of the data they were pretrained on.
% %
% However, we did not stress test these models for such ethical biases.
% %
% We request our users to be aware of these ethical issues in our dataset that might affect their models and evaluations.

% \paragraph{Evaluation Biases}
% We use certain pretrained models as metrics for evaluation including the BERTScore and SummaQA.
% %
% These metrics carry biases of the data they were trained on.
% %
% For example, they have been known to have bias associating professions with a particular gender. 

% \paragraph{Crowdsourcing}
% Workers were hired through the Amazon Mechanical Turk platform and offered an a hourly rate of approximately 12 USD. 
% % 
% To ensure the high quality of hired workers the following requirements were applied:
% HIT approval rate greater than or equal to 97\%,
% %
% number of HITs approved greater than or equal to 10000,
% %
% and located in one of the following English speaking countries: Australia, Canada, United Kingdom, and United States.


==> tables/old/sub-task1-results.tex <==
\begin{table*}[!htbp]
    \centering
    \small
    
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lrrrrrrrrrrrrr} 
    \toprule

    \textbf{Models} & $\textrm{R}_{1f}$ & $\textrm{R}_{2f}$ & $\textrm{R}_{Lf}$ & $\textrm{BS}_{P}$ & $\textrm{BS}_{R}$ & $\textrm{BS}_{F1}$ & $\textrm{LP_{p3c}}$ & $\textrm{SummaC_{ZS}}$ & $\textrm{Length}$ & $\textrm{Density}$ & $\textrm{Coverage}$ & $\textrm{1-grams}$ & $\textrm{2-grams}$ \\
    
    
    \midrule
    & & \multicolumn{11}{c}{\textbf{Baselines}} \\
    \midrule
    $LED_{1024} & 0.1413 & 0.0214 & 0.1329 & 0.4318 & 0.4697 & 0.4446 & 0.2684 & 0.2599 & 937 & 1.5149 & 0.7230 & 0.2886 & 0.7094 $\\
    $LED_{4096} & 0.1537 & 0.0221 & 0.1426 & 0.4232 & 0.4727 & 0.4420 & 0.2642 & 0.4718 & 866 & 2.9900 & 0.7617 & 0.2409 & 0.6096 $\\
    $LED_{16384} & 0.1487 & 0.0218 & 0.1385 & 0.4282 & 0.4928 & 0.4544 & 0.2221 & 0.4132 & 755 & 2.2112 & 0.7372 & 0.2532 & 0.6541 $\\ 
    \midrule
    
    & & \multicolumn{11}{c}{\textbf{Sub-Task 1 submissions}} \\
    \midrule
    $MHPK  & 0.2975 & 0.0789 & 0.2833 & 0.5303 & 0.5553 & 0.5410 & 0.1071 & 0.1562 & 1465 & 2.1802 & 0.7735 & 0.3055 & 0.6775 $  \\
    $LRL\_NC & 0.2643 & 0.0471 & 0.2436 & 0.4717 & 0.5264 & 0.4955 & 0.0669 & 0.3499 & 3345 & 12.6336 & 0.8336 & 0.1600 & 0.3457 $ \\
    
    
    \bottomrule
    \end{tabular}
    }
    \caption{
    Sub-task 1 results for the baselines and the submissions on the \textit{BookSumm-chapters} dataset.
    % Don't add newlines here.
    }
    \label{tab:sub-task1-results}
\end{table*}






==> tables/old/sub-task2-results.tex <==
\begin{table*}[!htbp]
    \centering
    \small
    
        \small
    
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lrrrrrrrrrrrrr} 
    \toprule

    \textbf{Models} & $\textrm{R}_{1f}$ & $\textrm{R}_{2f}$ & $\textrm{R}_{Lf}$ & $\textrm{BS}_{P}$ & $\textrm{BS}_{R}$ & $\textrm{BS}_{F1}$ & $\textrm{LP_{p3c}}$ & $\textrm{SummaC_{ZS}}$ & $\textrm{Length}$ & $\textrm{Density}$ & $\textrm{Coverage}$ & $\textrm{1-grams}$ & $\textrm{2-grams}$ \\
    
    
    \midrule
    & & \multicolumn{11}{c}{\textbf{Baselines}} \\
    \midrule
LED_{1024}                     & 0.1492 & 0.0146 & 0.1373 & 0.4298 & 0.4238 & 0.4258 & 0.2517 & 0.0000 & 903 & 1.1809 & 0.7021 & 0.3357 & 0.7485 \\
LED_{4096}                    & 0.1416 & 0.0130 & 0.1299 & 0.4245 & 0.4137 & 0.4179 & 0.2674 & 0.0000 & 877 & 1.3432 & 0.7311 & 0.3092 & 0.7273 \\
LED_{16384}                    & 0.1368 & 0.0125 & 0.1277 & 0.4322 & 0.3924 & 0.4099 & 0.2312 & 0.0000 & 551 & 1.4103 & 0.7266 & 0.3024 & 0.7211 \\
    \midrule
    
    & & \multicolumn{11}{c}{\textbf{Sub-Task 2 submissions}} \\
    \midrule
MovING\_scriptbase            & 0.4144          & 0.0823          & 0.3963          & 0.5163          & 0.5233          & 0.5194           & 0.0356                       & 0.0476              & 729               & 3.4398               & 0.8759               & 0.1621               & 0.4827                \\
UdS\_scriptbase               & 0.4285          & 0.1088          & 0.4125          & 0.5543          & 0.5410          & 0.5474           & 0.0587                       & 0.0323              & 883               & 1.3489               & 0.7778               & 0.2911               & 0.7346                \\
UdS\_base\_bs4\_0.2noisy      & 0.4634          & 0.1158          & 0.4405          & 0.5723          & 0.5680          & 0.5700           & 0.0372                       & 0.0250              & 791               & 1.2722               & 0.7502               & 0.3520               & 0.7636                \\
UdS\_base\_bs4\_Bitfit        & 0.4344          & 0.1091          & 0.4178          & 0.5533          & 0.5402          & 0.5465           & 0.0566                       & 0.0321              & 815               & 1.3475               & 0.7753               & 0.2879               & 0.7301                \\
UdS\_base\_bs4\_Bitfit\_Mix01 & 0.4580          & 0.1162          & 0.4376          & 0.5664          & 0.5601          & 0.5631           & 0.0459                       & 0.0316              & 770               & 1.3226               & 0.7590               & 0.3235               & 0.7457                \\
UdS\_base\_bs4\_Bitfit\_Mix10 & 0.4576          & 0.1158          & 0.4380          & 0.5690          & 0.5620          & 0.5653           & 0.0418                       & 0.0301              & 781               & 1.3194               & 0.7628               & 0.3167               & 0.7459                \\
UdS\_base\_bs4                & 0.4639          & 0.1152          & 0.4408          & 0.5703          & 0.5672          & 0.5686           & 0.0408                       & 0.0269              & 780               & 1.2733               & 0.7513               & 0.3456               & 0.7604                \\
UdS\_base\_bs5\_Bitfit        & 0.4316          & 0.1088          & 0.4151          & 0.5542          & 0.5414          & 0.5475           & 0.0567                       & 0.0309              & 838               & 1.3451               & 0.7774               & 0.2890               & 0.7327                \\
UdS\_base\_bs5\_Bitfit\_Mix01 & 0.4550          & 0.1149          & 0.4344          & 0.5664          & 0.5606          & 0.5634           & 0.0508                       & 0.0322              & 776               & 1.3344               & 0.7621               & 0.3205               & 0.7438                \\
UdS\_base\_bs5\_Bitfit\_Mix10 & 0.4553          & 0.1146          & 0.4353          & 0.5677          & 0.5619          & 0.5646           & 0.0435                       & 0.0295              & 777               & 1.3235               & 0.7596               & 0.3218               & 0.7462                \\
UdS\_base\_bs5                & 0.4604          & 0.1140          & 0.4369          & 0.5699          & 0.5668          & 0.5682           & 0.0410                       & 0.0281              & 783                & 1.2709               & 0.7493               & 0.3485               & 0.7649                \\

    
    
    \bottomrule
    \end{tabular}
    }%
    \caption{
    Sub-task 2 results for the baselines and the submissions on the \textit{Scriptbase} dataset.
    % Don't add newlines here.
    }
    \label{tab:sub-task2-results}
    

\end{table*}






==> tables/old/sub-task3-results.tex <==
\begin{table*}[htbp]
    % \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lrrrrrrrrrrrrrrrr} 
    \toprule

    \textbf{Models} & $\textrm{R}_{1f}$ & $\textrm{R}_{2f}$ & $\textrm{R}_{Lf}$ & $\textrm{BS}_{P}$ & $\textrm{BS}_{R}$ & $\textrm{BS}_{F1}$ & $\textrm{LP_{p3c}}$ & $\textrm{SummaC_{ZS}}$ & $\textrm{Length}$ & $\textrm{Density}$ & $\textrm{Coverage}$ & $\textrm{1-grams}$ & $\textrm{2-grams}$ \\
    
    
    \midrule
    & & \multicolumn{11}{c}{\textbf{Baselines}} \\
    \midrule
LED_{1024}                      & 0.1428          & 0.0154          & 0.1236          & 0.4100          & 0.4107          & 0.4052           & 0.0987                       & 0.0559              & 330               & 1.1440               & 0.7148               & 0.3060               & 0.7801                \\
LED_{4096}                      & 0.1694          & 0.0209          & 0.1501          & 0.4591          & 0.4752          & 0.4600           & 0.0304                       & 0.1052              & 188               & 1.4378               & 0.7343               & 0.2803               & 0.7314                \\
LED_{16384}                     & 0.1514          & 0.0170          & 0.1334          & 0.4485          & 0.4632          & 0.4489           & 0.0304                       & 0.1644              & 192               & 1.5474               & 0.7108               & 0.2904               & 0.7285                \\
    \midrule
    
    & & \multicolumn{11}{c}{\textbf{Sub-Task 3 submissions}} \\
    \midrule

inotum    & 0.2860          & 0.0624          & 0.2529          & 0.5934          & 0.5609          & 0.5750           & 0.0559                       & 0.0272              & 86                & 1.0321               & 0.6664               & 0.3715               & 0.8251                \\
team\_ufal            & 0.2469          & 0.0408          & 0.2300          & 0.5038          & 0.5590          & 0.5285           & 0.0406                       & 0.1282              & 289               & 2.0821               & 0.7127               & 0.2484               & 0.6498                \\
AMRTVSumm & 0.2307          & 0.0303          & 0.2106          & 0.4906          & 0.5344          & 0.5108           & 0.0138                       & 0.024               & 256               & 0.8789               & 0.6137               & 0.4924               & 0.8569                \\

    
    
    \bottomrule
    \end{tabular}
    }%
    \caption{
    Sub-task 3 results for the baselines and the submissions on the \textit{SummScreenFD} dataset.
    % Don't add newlines here.
    }
    \label{tab:sub-task3-results}
\end{table*}






==> tables/old/sub-task4-results.tex <==
\begin{table*}[htbp]
    % \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lrrrrrrrrrrrrrrrr} 
    \toprule

    \textbf{Models} & $\textrm{R}_{1f}$ & $\textrm{R}_{2f}$ & $\textrm{R}_{Lf}$ & $\textrm{BS}_{P}$ & $\textrm{BS}_{R}$ & $\textrm{BS}_{F1}$ & $\textrm{LP_{p3c}}$ & $\textrm{SummaC_{ZS}}$ & $\textrm{Length}$ & $\textrm{Density}$ & $\textrm{Coverage}$ & $\textrm{1-grams}$ & \textrm{2-grams} \\
    
    
    \midrule
    & & \multicolumn{11}{c}{\textbf{Baselines}} \\
    \midrule
$LED_{1024}$                         & 0.0727          & 0.0063          & 0.0652          & 0.4100          & 0.4107          & 0.4052           & 0.0304                       & 0.0905              & 984               & 0.9530               & 0.6302               & 0.3781               & 0.8379                \\
$LED_{4096}$                           & 0.0822          & 0.0062          & 0.0753          & 0.4122          & 0.4086          & 0.4057           & 0.0304                       & 0.0837              & 879               & 0.8457               & 0.5822               & 0.4091               & 0.8674                \\
$LED_{16384}$                          & 0.0722          & 0.0047          & 0.0656          & 0.4096          & 0.3916          & 0.3960           & 0.0304                       & 0.0800              & 885               & 0.7544               & 0.5430               & 0.4387               & 0.8931                \\ 

    \midrule
    
    & & \multicolumn{11}{c}{\textbf{Sub-Task 4 submissions}} \\
    \midrule

AdityaUpadhyay & 0.3921          & 0.0909          & 0.3794          & 0.5507          & 0.5550          & 0.5516           & 0.0625                       & 0.1133              & 316               & 1.9436               & 0.7618               & 0.2026               & 0.6688                \\
AMRTVSumm      & 0.3426          & 0.0717          & 0.328           & 0.5385          & 0.5318          & 0.5347           & 0.0152                       & 0.0499              & 259               & 1.1024               & 0.7291               & 0.3514               & 0.7931                \\

    
    
    \bottomrule
    \end{tabular}
    }%
    \caption{
    Sub-task 4 results for the baselines and the submissions on the \textit{SummScreenTMS} dataset.
    % Don't add newlines here.
    }
    \label{tab:sub-task4-results}
\end{table*}





